Breaking Down the Defenses: A Comparative Survey of Attacks on Large Language Models

Large Language Models (LLMs) have become a cornerstone in the field of Natural Language Processing (NLP), offering transformative capabilities in understanding and generating human-like text. However, with their rising prominence, the security and vulnerability aspects of these models have garnered significant attention. This paper presents a comprehensive survey of the various forms of attacks targeting LLMs, discussing the nature and mechanisms of these attacks, their potential impacts, and current defense strategies. We delve into topics such as adversarial attacks that aim to manipulate model outputs, data poisoning that affects model training, and privacy concerns related to training data exploitation. The paper also explores the effectiveness of different attack methodologies, the resilience of LLMs against these attacks, and the implications for model integrity and user trust. By examining the latest research, we provide insights into the current landscape of LLM vulnerabilities and defense mechanisms. Our objective is to offer a nuanced understanding of LLM attacks, foster awareness within the AI community, and inspire robust solutions to mitigate these risks in future developments.

==> sections/attack-objectives.tex <==
\section{\acb{The Underlying Objectives of LLM Attacks}}

\subsection{Evasion}
Evasion attacks in LLMs involve strategies where attackers manipulate input data to bypass filters or detection mechanisms, often without compromising the model's overall performance on benign inputs \cite{biggio2013evasion}\cite{dang2017evading}. These attacks are particularly concerning in contexts where LLMs are used for content moderation or sensitive decision-making.
Attackers can craft inputs that evade content filters, leading to the dissemination of harmful or inappropriate content. This raises significant concerns about the reliability of LLMs in regulated or sensitive environments ~\cite{carlini2020evading}.


\subsection{Poisoning}
Data poisoning involves altering the training data of an LLM, leading to manipulated model behavior. Such attacks can be particularly insidious as they can occur during the data collection phase, often going undetected until after deployment ~\cite{chen2017targeted}.
By adding carefully crafted data into the training set, attackers can influence the model's outputs, potentially leading to biased or harmful generated texts ~\cite{biggio2012poisoning}.


\subsection{Model Stealing}
Model stealing attacks aim to replicate the functionality of a proprietary LLM. Through such attacks, adversaries may gain unauthorized access to the model's capabilities, intellectual property, or even infer its training data ~\cite{tramer2016stealing, orekondy2019knockoff}. Attackers attempt to reverse-engineer the model's parameters or architecture, compromising its uniqueness and potentially leading to unauthorized reproductions ~\cite{correia2018copycat}.


\subsection{Model Inversion}
Model inversion attacks on LLMs aim to extract sensitive information from the model, such as details about the training data or specific inferences made by the model ~\cite{fredrikson2015model}. These attacks can potentially reveal personal or proprietary information that was included in the model’s training data, posing significant privacy concerns ~\cite{hitaj2017deep}.


\subsection{Operational Threats}
Operational threats refer to attacks that target the deployment and operational use of LLMs. These attacks can disrupt the service, lead to unauthorized access, or compromise the integrity of the model’s outputs.
Attackers may target the infrastructure supporting the LLM, leading to service outages or degraded performance \cite{barreno2010security}.
This involves gaining illicit access to the model, allowing attackers to manipulate outputs or steal sensitive data \cite{goodfellow2014explaining}.

We categorize attacks on LLMs based on two pillars i) based on access to model weights ii) based on attack vectors. We review 63 papers that encompass these pillars, and accordingly we provide a taxonomy of attacks on LLMs that will enable researchers to better understand the landscape.



==> sections/data-poisoning.tex <==
\subsection{Data Poisoning}
\label{subsec:Data Poisoning}
\hypertarget{data-poisoning}{}

\textbf{Universal attacks: }
"Forcing Generative Models to Degenerate Ones: The Power of Data Poisoning Attacks": This study highlights the impact of minimal poisoned data on generative models, particularly in natural language generation tasks, showing substantial performance degradation with slight data manipulation during fine-tuning.
"Concealed Data Poisoning Attacks on NLP Models": This paper focuses on covert data poisoning strategies in NLP models, detailing how small, concealed changes to training data can control model predictions, underscoring the subtlety and effectiveness of these attacks in manipulating language models.

\textbf{Domain specific attacks: } 

cite("Poisoning Scientific Knowledge Using Large Language Models") introduce "Scorpius," a model designed to generate malicious content to mislead scientific knowledge graphs, particularly in the biomedical domain, demonstrating the potential misuse of LLMs in specialized fields
cite("VonGoom: Transforming Data Poisoning in Large Language Models" discuss VonGoom), a method focusing on the strategic placement of a small number of inputs to deceive LLMs during training, particularly in prompt-specific attacks, showcasing its application across different contexts.

\textbf{Backdoor attacks: }

cite("Backdoor Activation Attack: Attack Large Language Models using Activation Steering for Safety-Alignment) presents a comprehensive study on adversarial attacks targeting the alignment of Large Language Models (LLMs). \vjb{The authors} introduce a method for universal activation attacks across different target alignments, using contrastive layer selection for effective intervention. The paper demonstrates the success of these attacks in compromising LLMs' adherence to \vjb{it's} intended guidelines, such as truthfulness and toxicity, by manipulating model components during inference.

cite("Composite Backdoor Attacks Against Large Language Models) focuses on developing stealthier backdoor attacks by employing multiple trigger keys in a composite manner. This approach is effective in both NLP and multimodal tasks, illustrating the capability to covertly introduce vulnerabilities into LLMs that serve as foundational models for various researches and services. The study highlights the increased sophistication in backdoor attack methodologies, emphasizing the need for vigilant defenses against such covert threats.

cite("Poisoning Scientific Knowledge Using Large Language Models") introduce "Scorpius," a model designed to generate malicious content to mislead scientific knowledge graphs, particularly in the biomedical domain, demonstrating the potential misuse of LLMs in specialized fields
cite("VonGoom: Transforming Data Poisoning in Large Language Models" discuss VonGoom), a method focusing on the strategic placement of a small number of inputs to deceive LLMs during training, particularly in prompt-specific attacks, showcasing its application across different contexts.





==> sections/evaluation.tex <==
\section{Evaluation} We evaluate various works in Table \ref{tab:llm-atttack}

\begin{table*}[]
\begin{tabular}{|p{1cm}|p{2cm}|p{2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1.5cm}|}
\hline
Category & Sub-Category & Paper Name  & Target Model  &  Attack Assumption   & Query-based Attack & Model-based Attack & Training Data-based Attack  & Dataset & Attack Success Rate & Text-based/ Image-based/ Audio-based \\ \hline
  \multirow{6}{*} {\rotatebox{90}{ {Prompt Injection}} }    &    Objective Manipulation          &    \cite{abdelnabi2023not}   &     GPT-3.5    &   B     &    \textcolor{green}{\ding{51}}                                   &            \textcolor{red}{\ding{53}}         &      \textcolor{green}{\ding{51}}              &                    &               &     \\  \cline{2-11}
    
         &      Prompt Leaking        &            &         &              &                                       &                     &                    &                    &            &       \\  \cline{2-11}
         &     Malicious Content Generation         &            &         &              &                                       &                     &                    &                    &    &  \\  \cline{2-11}
          &     Manipulating Training Data to Influence Prompt Injection         &            &         &              &                                       &                     &                    &                    &    &  \\  \cline{2-11}

        &     LLM Integrated Application         &            &         &              &                                       &                     &                    &                    &    &  \\  \cline{2-11}

        &     Prompt Manipulation Framework         &            &         &              &                                       &                     &                    &                    &    &  \\  \cline{2-11}
        &     Benchmarking         &            &         &              &                                       &                     &                    &                    &    &  \\ \hline
\end{tabular}
\label{tab:llm-attack}
\caption{Attack Assumption- (B)lack box, (G)ray box, and (W)white box}
\end{table*}
